What Guides Our Choices? Modeling Developers' Trust and Behavioral Intentions Towards GenAI

Generative AI (genAI) tools, such as ChatGPT or Copilot, are advertised to improve developer productivity and are being integrated into software development. However, misaligned trust, skepticism, and usability concerns can impede the adoption of such tools. Research also indicates that AI can be exclusionary, failing to support diverse users adequately. One such aspect of diversity is cognitive diversity -- variations in users' cognitive styles -- that leads to divergence in perspectives and interaction styles. When an individual's cognitive style is unsupported, it creates barriers to technology adoption. Therefore, to understand how to effectively integrate genAI tools into software development, it is first important to model what factors affect developers' trust and intentions to adopt genAI tools in practice? We developed a theoretically grounded statistical model to (1) identify factors that influence developers' trust in genAI tools and (2) examine the relationship between developers' trust, cognitive styles, and their intentions to use these tools in their work. We surveyed software developers (N=238) at two major global tech organizations: GitHub Inc. and Microsoft; and employed Partial Least Squares-Structural Equation Modeling (PLS-SEM) to evaluate our model. Our findings reveal that genAI's system/output quality, functional value, and goal maintenance significantly influence developers' trust in these tools. Furthermore, developers' trust and cognitive styles influence their intentions to use these tools in their work. We offer practical suggestions for designing genAI tools for effective use and inclusive user experience.

==> _tex_folder/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> _tex_folder/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.79.  Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.80.  New journals: DLT, FAC


==> sec/7.Threat.tex <==
% \vspace{-2px}
% \pagebreak



% \noindent\textbf{\textit{Statistical conclusion}}: 
% All statistical methods and tests used in our analysis follow the latest guidelines in our field \cite{russo2021pls}. We addressed potential threats to model validity, including common method variance, unobserved heterogeneity, and model overfitting, with our analyses indicating the absence of these issues in our study.


==> sec/TODO.tex <==
Vocab check:
genAI tools, genAI





----------------------------------------------
1. How PICSE -> trust. How trust -> BI->use. (Added in RQ1 and RQ2)
2. Motivations, Challenges, Risks (Rq4)
3. How 2 explains 1. (Rq4)
4. [dropped] Occupational demographics (Phase, Exp, AI familiarity:
    How it affects 1, 2 ()R3
5. How CS associates with #2. Similarities and differences across SDLC. 
6. How PICSE factors vary with 
    - Cogn. Style
    - phase
    - occupational demg. 
Another contribution is validating PICSE. 
------------------------------------------------
1. PICSE validation + GM -> Trust + Intentions
2. 1 + MGA (Job role, Gender, Experience) + IPMA + Qual Analysis (C, R, M) and How it effects trust. Analysis (sim. + diff across job roles, gender, experience)
3. Same model but for students and gradients across devs, students.



Discussion text
- Aligning AI to human aspects
- Guidelines and design strategies to foster trust. 

Points
-> Theoretical contributions
    - \textbf{Validated questionnaire}
    - Associations
    - What creates trust in genAI and how trust and cognitive styles combine to influence adoption.
        - What PICSE components really matter and by how much. How cognitive styles matter to adoption and not every thing is a hype. Inclusive building is necessary. People might use it due to peer pressure anyways but if styles not supported they will suffer. We want these factors to not matter but it will only be so if inclusive AI. Use these insights to scope appropriate trust and not to increase (only advised to increase/align if looking at warranted trust through trustworthiness).

    -> Trust is contractual and contextual
    - \textbf{Contextual}: human might feel positive trust toward an AI system w.r.t certain contexts, and simultaneously feel mistrust and distrust when other context are involved. 
        - Context is SE (\textbf{finer context is job roles}, which we couldnt capture in this work and is \textbf{open for future work})
        - Contractual 
        -Source reputation and community shown to matter but unwarranted. 

-> Implications for research
    - Policy implications
    - Inclusive AI
    - AI Alignment and governance (accountability, timing of intervention, not loss of agency)

-> Implications for practice
    - Warranted trust
        - How to \textbf{promote warranted trust} (transparency and XAI can help how? - see formalization in trust paper)
        - XAI should enable user to know whether, when, and why to trust upon and to what extent (rely/not rely/rely with caution).
    - Design principles/Guidelines to foster trust
    - Goal alignment (capabilities will improve anyhow)

==> sec/discussion-old.tex <==
% Implications for associations
\subsection{Implications (Rudy Here)}

\textbf{\textit{1) Foster appropriate trust in genAI tools by promoting warranted trust and minimizing unwarranted trust in these tools.}}

% ** \boldification{Warranted trust forms are based on system's actual trustworthiness; while unwarranted is based on non-substantive factors. Unwarranted attributes can induce trust, and may be detrimental for developers who overestimate the capabilities of these tools in critical tasks.}

Warranted trust refers to the accurate calibration of trust, reflecting a system's trustworthiness \cite{jacovi2021formalizing}. Essentially, trust is warranted when users' confidence in a tool aligns with its true capabilities. Conversely, unwarranted trust is influenced by factors that do not genuinely represent a system's reliability, such as its reputation or anthropomorphic features \cite{jensen2020role}. These attributes can mislead users into overestimating the system's capabilities, potentially leading to detrimental outcomes in high-impact scenarios or critical tasks \cite{pearce2022asleep}.

% \boldification{Thus, calibration is needed between trust and trustworthiness. This helps scope appropriate expectations about quality and value (which are both related to trust)}

Therefore, calibrating users' trust to match a system's true capabilities is essential. This alignment allows users to form realistic expectations about the \textit{system's quality} and appropriately assess its \textit{functional value} \cite{wischnewski2023measuring, amershi2019guidelines}. Our findings suggest that both system quality and functional value significantly influence developers' trust in genAI tools.  Increasing the reliability and overall quality of system output, and also making the utility of the system more transparent both promote higher levels of trust in these of genAI tools.


% \boldification{The key is to design tools that provide explicit cues. Design should emphasize transparency thru explanability.} 

Designing for warranted trust involves creating interfaces that provide explicit, accurate cues about a system's capabilities and limitations.  This approach is emphasized in several AI design guidelines \cite{amershi2019guidelines, GoogleGuidelines} aimed at supporting HAI interactions. To achieve this, toolsmiths should prioritize transparency in AI’s behavior (e.g., scoping of services in uncertainty \cite{amershi2019guidelines}) and its outputs (e.g., confidence scores \cite{wang2023investigating}).
% 
% \boldification{XAI can inform true trustworthiness and incite appropriate trust.}
 
Moreover, explainability is pivotal in calibrating trust. It serves two key functions: (a) it clarifies the trustworthiness of AI by elucidating its reasoning process \cite{jacovi2021formalizing}, and (b) fosters appropriate trust in AI by enabling users to anticipate its behavior through informed signals \cite{wischnewski2023measuring}, while revealing any flaws or inconsistencies in its logic.
% \boldification{However, explanations might cause info overload. Thus, timing of intervention is crucial to ensure users maintain trust without cognitive overload.}
However, it is important to manage the presentation of explanatory features to avoid information overload \cite{wang2023investigating}. While detailed indicators can guide actions, excessive information can overwhelm users, leading to biases or misinterpretations. Effective design should, therefore, support timely interventions \cite{jacovi2021formalizing} that provide information about output quality and utility only as needed or on-demand, ensuring users maintain appropriate trust in the system without experiencing cognitive overload.


\textit{\textbf{2) Design AI to maintain human goals}}


% Goal alignment manifests trust - it is important for cognitive flow, making users perceive AI as a cognitive collaborator. 

% Trust in AI is context-dependent; it varies across different tasks and contexts. Developers may find AI trustworthy for specific functions, such as code generation, but less reliable for tasks like debugging, and thereby less trustworthy. Recognizing this variability, goal maintenance and control in designing AI becomes crucial to foster trust in these tools.  

% This is where goal maintenance and control become important. 

% To design for goal maintenance, alignment between AI behavior and human goals are important. 
% Ensuring that AI systems maintain user goals is fundamental to building trust. This goes beyond superficial preferences or like/dislike responses. It requires a deep integration into the  reasons behind users' trust or distrust. Why did users reject an AI's suggestion? What underlying goals were not met? Capturing these insights is key to refining AI behavior.

% To achieve goal maintenance, AI systems must be designed to not only acknowledge but also affirm/adhere to user goals. This involves understanding and supporting the user's intentions and ensuring the AI's actions are consistently aligned with these intentions. Such alignment reinforces trust, as users see the AI as a reliable partner that upholds their objectives.

% Further, designing for control is another aspect - AI while maintaining goals, should support users in maintaining decision-making agency, and must be accountable to the human for its actions. 


\textit{\textbf{3) Design strategies should promote fairness in HAI-UX through inclusivity}}


% Ideas about fairness is receiving attention, but usually refers to data or algorithmic fairness - these ideas are also relevant in hai-ux fairness.

% Inclusivity is crucial for fairness in HAI-UX. When an AI product leads to disadvantageous outcomes for a particular group of users (e.g., risk averse), then that product is not inclusive to that group. 


% Design strategies should thus priortize inclusivity. In our paper, we scope this discussion to inclusitivity of users' cognitive styles from the GenderMag method. ignoring cognitive styles can lead to exclusion and unfair experiences.

% Incorporating cognitive styles into products' HAI-UX can sometimes point out where and why mismatches are arising between a group of users and an AI product.

% To do so, genAI design should be adaptive to cognitive styles. This starts by first capturing the cognitive styles, which can be done in user profiling using the validated scale. 

% GenAI can then adapt its behavior based on the cognitive styles of the user. For example, users can have diverse risk attitudes. For the risk averse ones, design should prioritize transparency and explainability -> important for the user to know when and to what extent the AI can be trusted, thus leading to their positive behavioral intentions. 






==> sec/leftover-text.tex <==
Overfitting analysis:

Given that high $R^2$ and $f^2$ values might raise concerns about potential overfitting (where the model inadvertently learns noise from the training data, compromising its ability to predict unseen data), we tested for model overfitting, adhering to recommended approaches presented in previous studies. The associated code can be found in the supplemental package.

First, we analyzed model residuals to assess the appropriateness of the model fit. Residuals represent the differences between the observed and predicted values for dependent variables and are expected to be randomly scattered around 0 in a well-specified model. This suggests that the errors are random and the model is correctly specified. Figures X and Y present the plots for the residuals against the predicted values for the `trust' and `behavioral intention' constructs, respectively. The residuals are indeed randomly scattered, suggesting that the model errors are random.

Next, we triangulated the lack of overfitting using train-test split and cross-validation: (1) We performed an 80-20 split, where the model was trained on 80\% of the data and tested on the remaining 20\%. The performance was assessed using the mean squared error (MSE), where low values indicate a good fit. The MSE values for the trust and intention constructs were 0.317 and 0.381, respectively, both of which fall within the accepted MSE range. (2) We implemented k-fold cross-validation with k set to 5, in line with recommended practices in prior studies. The data was divided into 5 subsets, and the model was trained and tested 5 times, each time on a different subset of the data. The performance was again assessed using MSE. The mean MSE for cross-validation were 0.323 and 0.377 for the trust and intention constructs, respectively. These values are close to the test MSE, suggesting that the model is not overfitting the data.

Overall, the analyses suggest that our model is generalizing effectively to unseen data, confirming the lack of model overfitting.




==> sec/outline.tex <==
Questions:
SYSTEM/OUTPUT QUALITY	

S2	genAI_technology_is_well_crafted_with_no_visual_issues
S3	genAI_technology_clearly_takes_care_of_important_matters_like_security_and_privacy
S4	genAIs_outcomes_seem_consistently_correct
S5	genAI_tools_run_smoothly_with_no_or_minimal_performance_issues
E3	genAIs_contributions_match_my_style
		
FUNCTIONAL VALUE	
I3	I_feel_I_can_learn_from_using_genAI_technology
P3	There_are_potential_benefits_of_using_genAI_technology


Intro

Background
- CS
- PICSE
- Trust
- Behavioral Intentions

Theory Development

For each RQ from 1 to 3:
    Text for belief (Support for Hypothesis)
    Hypothesis

Research Design

    Measurement model (explain each construct and respective indicators, also where they came from)
    
    Data Collection
    * Designing the instrument (here the quest):
    * Piloting the questionnaire
    * Recruiting participants
    * Sample Analysis
    
    Quantitative Analysis
    * Using PLS and why
    
    Qualitative Analysis
    * Using open coding (inductive) for open questions

Measurement Validity
* Convergent Validity
* Internal Consistency Reliability
* Discriminant Validity
* Collinearity Assessment

Results
Evaluating the Structural model: Antecedents to trust and intentions
RQ1 and RQ2
* Path Coefficients and Significance
* Model Evaluation
* Importance-Performance Map

Trust and Intention to Use GenAI across demographics (MGA, IPMA)
RQ3
* Group Creation
* Evaluation of Measurement Invariance of Composite Models (MICOM)
* Groups Comparison and Analysis


Qualitative stuff (heading for now)
RQ4



\subsection{Evaluating the Structural model}
\subsubsection{Path Coefficients and Significance}
\subsubsection{Model Evaluation (R, F, Q)}
\subsubsection{Cluster Analysis}
\subsubsection{Common Method Bias and Overfitting}
% \subsubsection{Importance-Performance Map}
% \subsection{Motivations, Challenges, Risks}

% \subsection{Trust and Intention to Use GenAI across demographics}
% RQ3
% \subsubsection{Group Creation}
% \subsubsection{Evaluation of Measurement Invariance of Composite Models (MICOM)}
% \subsubsection{Groups Comparison and Analysis}

==> table/cluster.tex <==

\begin{table}[!tb]
\centering
\scriptsize
\caption{FIMIX - Optimal number of segments}
\label{tab:fimix}

\robustify{\bfseries}
\robustify{\itshape}
\sisetup{
    mode=text,
    group-digits = false ,
    detect-all=true,
    input-signs ={-},
    input-symbols = ( ) [ ] - + *,
    detect-weight=true, 
    detect-family=true,
    table-format=3.3,
    add-decimal-zero=false, %% doesn't seem to work :-(
    add-integer-zero=false,
    round-mode=places,
    round-precision=2, %% change this for precision.
    parse-numbers = true
}


\begin{tabular}{p{0.8cm}p{2cm}SS[table-format=4.3]}
\toprule
Group & Criterion & \bfseries{1-Segment} & {2-Segment}\\
\midrule
\multirow{2}{=}{1}& AIC3 & 1483.821 & \itshape 1480.38 \\
& CAIC & \itshape 1542.85 & 1601.91 \\ 
\midrule
\rowcolor{vlightgray} 

\cellcolor[gray]{.9} & \bfseries AIC4 & \bfseries \textit{1500.81}	& 1515.38 \\
\rowcolor{vlightgray} 
\multirow{-2}{=}{\cellcolor[gray]{.9}2}& \bfseries BIC & \bfseries \textit{1525.85} & 1566.91 \\
\midrule 
3 & EN & 0 & 0.324 \\
\bottomrule
\end{tabular}
\vspace{-5mm}
\end{table}

==> table/demographics2.tex <==
\begin{table}[!t]
\scriptsize
\centering
\caption{Respondent Demographics (n=238)}
\label{tab:demographics}
\vspace{-8px}
\robustify{\bfseries}
% \sisetup{
%     mode=text,
%     group-digits = false ,
%     input-symbols = ( ) [ ] - + *,
%     detect-weight=true, 
%     detect-family=true,
%     table-format=0.2,
%     add-decimal-zero=false, %% doesn't seem to work :-(
%     add-integer-zero=false,
%     round-mode=places, 
%     round-precision=1, %% change this for precision.
%     parse-numbers = true
% }

\begin{tabular}{llrl}
\toprule
\multirow{4}{*}[-2mm]{\rotatebox{90}{\textbf{Gender}}} &                         Attribute &   N & Percentage \\
\midrule
                &                               Man & 186 &      78.2\% \\
                &                             Woman &  39 &      16.4\% \\
                &      Non-binary or gender diverse &   6 &       2.5\% \\
                &                 Prefer not to say &   7 &       2.9\% \\
\midrule
\multirow{6}{*}[-2mm]{\rotatebox{90}{\textbf{Residence}}} 
                &                     North America & 129 &      54.2\% \\
                &                            Europe &  55 &      23.1\% \\
                &                              Asia &  33 &      13.8\% \\
                &                            Africa &   9 &       3.8\% \\
                &                     South America &   8 &       3.4\% \\
                &                   Pacific/Oceania &   4 &       1.7\% \\
\midrule
\multirow{4}{*}[-2mm]{\rotatebox{90}{\textbf{SE Experience}}} 
                &                         1-5 years &  57 &      23.9\% \\
                &                        6-10 years &  50 &      21.0\% \\
                &                       11-15 years &  52 &      21.9\% \\
                &                     Over 15 years &  79 &      33.2\% \\
\midrule
\multirow{12}{*}[-2mm]{\rotatebox{90}{\textbf{SE Responsibilities}}} 
                &                Coding/Programming & 223 &      93.7\% \\
                &                       Code Review & 192 &      80.6\% \\
                &                     System Design & 148 &      62.1\% \\
                &                     Documentation & 110 &      46.2\% \\
                &             Maintenance \& Updates & 108 &      45.4\% \\
                & Requirements Gathering \& Analysis & 108 &      45.4\% \\
                &          Performance Optimization & 107 &      44.9\% \\
                &       Testing \& Quality Assurance &  98 &      41.2\% \\
                &                    DevOps/(CI/CD) &  90 &      37.8\% \\
                &     Project Management \& Planning &  53 &      22.3\% \\
                &  Security Review \& Implementation &  46 &      19.3\% \\
                &  Client/Stakeholder Communication &  32 &      13.5\% \\
\bottomrule
\end{tabular}
\vspace{-6mm}
\end{table}


==> table/htmt.tex <==
\begin{table*}[h]
\centering
\caption{Heterotrait-Monotrait ratio of correlations (HTMT) of the model}
\begin{tabular}{lccccccccc}

\hline
 & \textbf{BI} & \textbf{EoU} & \textbf{FV} & \textbf{IP} & \textbf{LS} & \textbf{M} & \textbf{RT} & \textbf{SE} & \textbf{SOQ} \\ \hline
Behav. Intention (BI) &  &  &  &  &  &  &  &  &  \\
Ease of use (EoU) & 0.631 &  &  &  &  &  &  &  &  \\
Functional Value (FV) & 0.779 & 0.611 &  &  &  &  &  &  &  \\
Info Processing (IP) & 0.064 & 0.27 & 0.1 &  &  &  &  &  &  \\
Learning Style (LS) & 0.412 & 0.167 & 0.473 & 0.326 &  &  &  &  &  \\
Motivations (M) & 0.656 & 0.515 & 0.781 & 0.273 & 0.633 &  &  &  &  \\
Risk Tolerance (RT) & 0.664 & 0.366 & 0.561 & 0.127 & 0.517 & 0.791 &  &  &  \\
Self-Efficacy (SE) & 0.528 & 0.509 & 0.536 & 0.27 & 0.372 & 0.698 & 0.505 &  &  \\
System/Output Quality (SOQ) & 0.686 & 0.646 & 0.635 & 0.156 & 0.262 & 0.573 & 0.226 & 0.283 &  \\
Trust (T) & 0.762 & 0.585 & 0.664 & 0.169 & 0.286 & 0.649 & 0.394 & 0.333 & 0.752 \\ \hline
\end{tabular}
\label{table:correlation_matrix}
\end{table*}
